Grace periods in comparative effectiveness studies of sustained treatments

Researchers are often interested in estimating the effect of sustained use of a treatment on a health outcome. However, adherence to strict treatment protocols can be challenging for individuals in practice and, when non-adherence is expected, estimates of the effect of sustained use may not be useful for decision making. As an alternative, more relaxed treatment protocols which allow for periods of time off treatment (i.e. grace periods) have been considered in pragmatic randomized trials and observational studies. In this article, we consider the interpretation, identification, and estimation of treatment strategies which include grace periods. We contrast natural grace period strategies which allow individuals the flexibility to take treatment as they would naturally do, with stochastic grace period strategies in which the investigator specifies the distribution of treatment utilization. We estimate the effect of initiation of a thiazide diuretic or an angiotensin-converting enzyme inhibitor in hypertensive individuals under various strategies which include grace periods.

==> Extra/Tables/clinical_examples.tex <==
\begin{singlespace}
\begin{footnotesize}
\setlength{\tabcolsep}{5pt}
\begin{longtable}{ 
    P{15cm}
  }
\caption{Examples of natural and stochastic grace period treatment strategies with various values of $m$}\\ 

\underline{Natural grace period strategies} \\
\\
1. Individuals with clinical depression are assigned to receive cognitive behavioural therapy once every month, but they are allowed to skip their monthly session whenever they would prefer to, so long as they never skip more than $m=2$ in a row. \\
\\
2. Individuals with ulcerative colitis are prescribed infliximab to be taken every 8 weeks, but they are allowed to miss an infusion so long as they never miss more than $m=1$ in a row. \\
\\
3. Individuals with a history of breast cancer are assigned to take tamoxifen daily for 5 years, except they are allowed to miss a pill every day so long as they never miss more than $m=7$ in a row. \\
\\
4. Individuals with type II diabetes are treated with metformin. Each time they go to the pharmacy to receive medication, they are given exactly 1 month's supply. They are to receive medication every month, but they are allowed to miss dispensations so long as they never miss more than $m=2$ in a row. \\
\\
5. Individuals with hypertension are treated with a thiazide diuretic. They are given variable dispensation lengths - some receive 30 days of medication each time they go to the pharmacy, some 60 days, some 90 days, etc. They are to go to the pharmacy as often as they need to such that they have medication each month, but they are allowed up to $m=3$ months in a row where they do not have any medication. That is, if they go 3 months in a row without having medication, they must go to the pharmacy and receive medication. \\
\\
6. Individuals with hyperlipidemia are treated with a statin. They receive prescriptions for medication from their physician. They are to receive a prescription at the start of every 3-month study block, but they are allowed to miss getting a prescription so long as they do not miss more than $m=2$ in a row. \\
\\
\\

\underline{Stochastic grace period strategies} \\
\\
1. Individuals with clinical depression are assigned to receive cognitive behavioural therapy. The investigator flips a coin for each individual at the start of every month. If the coin comes up heads, the individual receives therapy. If tails, they do not receive therapy unless they have gone $m=2$ months in a row without getting therapy (because of prior coin flips) in which case the investigator ignores the coin and provides therapy. \\
\\
2. Individuals with ulcerative colitis are prescribed infliximab. The investigator flips a coin for each individual at the start of each 8 week study block. If the coin comes up heads, the individual is administered an infusion. If tails, they are not administered an infusion unless they were not administered an infusion in the last study block ($m=1$) due to the prior coin flip, in which case the investigator ignores the coin and administers an infusion. \\
\\
3. Individuals with a history of breast cancer are treated with tamoxifen for 5 years. Every day, they are to roll a 6-sided dice. If the result of the dice roll is a 3 or higher, they take a pill. If the result of the dice roll is a 1 or 2, then they don't take a pill unless they have missed taking a pill for the past $m=7$ consecutive days (due to prior dice rolls), in which case they ignore the dice and take a pill. \\
\\
4. Individuals with type II diabetes are treated with metformin. Each time they go to the pharmacy to receive medication, they are given exactly 1 month's supply. Every month, the investigator rolls a 4-sided dice for each individual. If the result of the dice roll is a 2 or higher, then the individual is to go to their pharmacy and receive medication. If the result of the dice roll is a 1 then the individual is not to receive medication unless they have gone $m=2$ consecutive months without medication (due to prior dice rolls) in which case they ignore the dice and go receive medication. \\
\\
5. Individuals with hypertension are treated with a thiazide diuretic. They are given variable dispensation lengths - some receive 30 days of medication each time they go to the pharmacy, some 60 days, some 90 days, etc. Whether they have medication in a given month depends on the roll of a 4-sided dice. If the result of the dice roll is a 2 or higher, then they are to have medication in that month. If the result of the dice roll is a 1 then they are not to have medication in that month unless it has been $m=3$ consecutive months without having medication in which case they ignore the dice and receive medication. \\
\\
6. Individuals with hyperlipidemia are treated with a statin. They receive prescriptions for medication from their physician. At the beginning of each 3-month study block the investigator flips a coin. If the result is heads, then the individual is given a prescription. If the result is tails then the individual is not given a prescription unless they have not been given prescriptions in both of the last $m=2$ study blocks (due to prior coin flips) in which case the investigator ignores the coin and provides a prescription. \\
\\

\bottomrule
\label{tab:clinical_example}
\end{longtable}
\end{footnotesize}
\end{singlespace}
